SciAssess: Benchmarking LLM Proficiency in Scientific Literature Analysis

Recent breakthroughs in Large Language Models (LLMs) have revolutionized scientific literature analysis. However, existing benchmarks fail to adequately evaluate the proficiency of LLMs in this domain, particularly in scenarios requiring higher-level abilities beyond mere memorization and the handling of multimodal data. In response to this gap, we introduce SciAssess, a benchmark specifically designed for the comprehensive evaluation of LLMs in scientific literature analysis. It aims to thoroughly assess the efficacy of LLMs by evaluating their capabilities in Memorization (L1), Comprehension (L2), and Analysis \& Reasoning (L3). It encompasses a variety of tasks drawn from diverse scientific fields, including biology, chemistry, material, and medicine. To ensure the reliability of SciAssess, rigorous quality control measures have been implemented, ensuring accuracy, anonymization, and compliance with copyright standards. SciAssess evaluates 11 LLMs, highlighting their strengths and areas for improvement. We hope this evaluation supports the ongoing development of LLM applications in scientific literature analysis. SciAssess and its resources are available at \url{https://github.com/sci-assess/SciAssess}.

==> chapters/backups/0_abstract.tex <==
\begin{abstract}

% Recent breakthroughs in Large Language Models (LLMs) have revolutionized natural language understanding and generation, sparking significant interest in applying them to scientific literature analysis. 
Recent breakthroughs in Large Language Models (LLMs) have revolutionized scientific literature analysis. 
However, existing benchmarks fail to adequately evaluate the proficiency of LLMs in this domain, particularly in scenarios requiring higher-level abilities beyond mere memorization and the handling of multimodal data.
In response to this gap, we introduce SciAssess, a benchmark specifically designed for the comprehensive evaluation of LLMs in scientific literature analysis. 
It aims to thoroughly assess the efficacy of LLMs by evaluating their capabilities in Memorization (L1), Comprehension (L2), and Analysis \& Reasoning (L3). 
It encompasses a variety of tasks drawn from diverse scientific fields, including biology, chemistry, material, and medicine.
To ensure the reliability of SciAssess, rigorous quality control measures have been implemented, ensuring accuracy, anonymization, and compliance with copyright standards. 
SciAssess evaluates 11 LLMs, highlighting their strengths and areas for improvement. 
We hope this evaluation supports the ongoing development of LLM applications in scientific literature analysis.
SciAssess and its resources are available at \url{https://anonymous.4open.science/r/SciAssess-2D14}.

\end{abstract}


==> chapters/backups/1_introduction.tex <==
\section{Introduction}
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/overview.pdf} 
  \vspace{-16pt}
  \caption{Overview of SciAssess. It spans over 4 sub-domains and encompasses 28 tasks.}
  \vspace{-12pt}
  \label{fig:overview}
\end{figure}
% LLM评估的重要性，理解模型性能边界，促进进步
Recent advances in Large Language Models (LLMs), such as GPT-4 \cite{gpt4}, Gemini \cite{gemini}, and Llama \cite{llama}, have attracted considerable attention due to their profound capabilities in natural language understanding and generation \cite{gpt-4-eval}. 
Evaluating these models is crucial for exploring their capability boundaries and limitations, thereby driving technological advancements.
In response, a variety of benchmarks tailored for LLMs have been proposed for extensive evaluation, covering a wide range of skills \cite{bm-2,bm-3} and diverse tasks \cite{bm-4, bm-5}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/radar_plot_full_sciassess_06122024.png}
    \vspace{-16pt}
    \caption{Performance overview of leading open and closed source LLMs on SciAssess. Each column represents a scientific domain. LLMs are evaluated on multiple tasks within each domain, with task details provided in Table \ref{tab:benchmark-stat}. For closed source LLMs (first row), GPT-4o and GPT-4 are the leading models. For open source LLMs (second row), Llama3 and Qwen2 emerge as the top models.}
    \vspace{-12pt}
    \label{fig:performance-overview}
\end{figure*}

% Specifically, LLMs have shown great potential in enhancing researchers' efficiency and productivity in scientific literature analysis \cite{science-llm}. Applications such as literature summarization and knowledge extraction have seen practical deployments \cite{scientific-literature-llm}. We categorize the ability of a literature analysis assistant into three level \cite{2009Krathwohl}: (1) \textbf{Memorization (L1)}: LLMs are able to accurately answer common factual questions across various scientific fields; (2) \textbf{Comprehension (L2)}: LLMs can identify, extract, and understand the core content of provided documents; and (3) \textbf{Analysis \& Reasoning (L3)}: LLMs can integrat extracted information with the existing knowledge base to perform logical reasoning and analysis.

Despite LLMs not yet fully replacing scientific researchers in generating creative discoveries, they have demonstrated substantial potential in enhancing researchers' efficiency in scientific literature analysis \cite{science-llm}. 
Specific applications such as automatic literature summarization and knowledge extraction have seen practical deployments, significantly boosting researchers' productivity and expanding the range of literature that can be effectively utilized \cite{scientific-literature-llm}.
Inspired by Bloom's Taxonomy \cite{taxonomy}, we systemize the requirements for scientific literature analysis assistants into three progressive levels: (1) \textbf{Memorization (L1)}: Establishing an extensive foundational knowledge base to accurately address common factual questions in various scientific domains; (2) \textbf{Comprehension (L2)}: Identifying, extracting, and understanding the core content of provided documents; and (3) \textbf{Analysis \& Reasoning (L3)}: Integrating extracted information with the existing knowledge base to perform logical reasoning and analysis.

Existing comprehensive LLMs benchmarks, such as MMLU \cite{mmlu}, include some tasks related to scientific data. However, these sub-tasks have two limitations: (1) they mostly focus on Memorization, neglecting higher-level abilities such as L2 and L3; (2) these tasks lack the evaluation of various multi-modal inputs (\eg charts, molecular structures, and tables), which are crucial in scientific literature. 

% To fill these gaps, we introduce \textbf{SciAssess} (\cf Figure \ref{fig:overview}) -- a new benchmark specifically designed measuring the ability of LLMs on scientific literature analysis. Our benchmark has the following features:

% Existing commonly-used LLM benchmarks, such as MMLU \cite{mmlu}, CMMLU \cite{cmmlu}, and Xiezhi \cite{xiezhi}, encompass a wide range of subjects, including scientific subsets.
% Nevertheless, we identify two limitations of them in evaluating LLMs' capabilities in scientific literature analysis: (1) when adopted in scientific literature analysis, their questions mostly focuses on Memorization (L1), neglecting higher-level abilities such as Comprehension (L2) and Analysis \& Reasoning (L3); and (2) The assessment of multimodal content interpretation (\eg charts, molecular structures, and tables), which often contain crucial information in scientific literature, is inadequate. 
% Consequently, there is a critical need for more specific LLM benchmarks that accurately reflect the complexity and specificity of scientific literature analysis.

In light of these existing limitations, we introduce \textbf{SciAssess} (\cf Figure~\ref{fig:overview}) -- a benchmark specifically designed for scientific literature analysis. 
SciAssess not only broadens the evaluation scope to encompass a wider range of LLM capabilities but also extends beyond text to include the extraction and interpretation of multimodal contents.
Moreover, meticulous design is essential to creating evaluations that yield deep insights, ensure fairness across different LLMs. 
Consequently, SciAssess is founded on three critical considerations:

\textbf{Model Ability.} A benchmark must clearly delineate the desired capabilities and model the intrinsic relationships among them, facilitating a diagnostic understanding.
Thus, SciAssess evaluates across three progressive levels (\ie Memorization (L1), Comprehension (L2), and Analysis \& Reasoning (L3)) and five modalities (\ie texts, charts, chemical reactions, molecular structures, and tables).
Consequently, SciAssess yields nuanced and informative evaluation outcomes, pinpointing specific aspects where the examined models may fall short.
    
\textbf{Scope \& Task.} Benchmarks should encompass a broad array of scientific domains to ensure comprehensiveness. 
Within each domain, the selected tasks must authentically represent the typical challenges and scenarios characteristic of that field.
Consequently, SciAssess spans over 4 sub-domains (\ie biology, chemistry, material, and medicine) and encompasses 28 tasks, each carefully suggested or designed by domain experts according to their professional experience.

\textbf{Scale \& Quality Control.} The scale and quality of the benchmark must be impeccable to serve as a dependable basis for deriving accurate, actionable, and applicable insights. 
SciAssess contains 6,938 questions in total to ensure adequate scale.
Each question is transformed from existing datasets or manually curated by domain experts hired by us \footnote{All data collection, annotation, and quality control tasks were carried out by the authors (who are also employees of the company) as part of their job responsibilities, and therefore, they were not provided with any additional compensation.}.
Subsequently, expert cross-validation is performed to ensure correctness and reliability. 

% 期望揭示出当前的llm在科学领域的性能，以进一步提升llm在该领域的能力
Overall, SciAssess aims to reveal the performance of LLMs as a scientific literature analysis assistant, thereby identifying their strength and weaknesses. 
% Following this, our objective is to promote the evolution of LLMs, ensuring they are not only better skilled at navigating scientific literature but also more capable of aiding the progress of research in diverse scientific fields.
The insights gained from SciAssess could hopefully catalyze further enhancing the capabilities of LLMs in scientific literature analysis, ultimately contributing to the acceleration of scientific discovery and innovation.

==> chapters/backups/2_benchmark.tex <==
\section{Benchmark Dataset}

\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{>{\centering\arraybackslash}m{1.1cm} >{\centering\arraybackslash}p{3.2cm} >{\centering\arraybackslash}p{0.6cm} >{\centering\arraybackslash}p{1.15cm} >
{\centering\arraybackslash}p{0.8cm} >
{\centering\arraybackslash}p{2.5cm} >{\centering\arraybackslash}p{2cm} >{\centering\arraybackslash}p{1.25cm}
}
\toprule
Domain & Task & Ability & \# Questions & Context & Question Type & Metric & Modality \\
\noalign{\vskip -1pt}\midrule\noalign{\vskip -1pt}
\multirow{4}{1.1cm}{\centering Fundamental Science} & \textcolor{gray}{MMLU (science)} & L1 & 2,091 & & Multiple Choice & Accuracy & Text only \\
 & \textcolor{gray}{CMMLU (science)} & L1 & 1,700 & & Multiple Choice & Accuracy & Text only   \\
 & \textcolor{gray}{Xiezhi-Ch (science)} & L1 & 2,882 & & Multiple Choice & Accuracy & Text only \\
 & \textcolor{gray}{Xiezhi-En (science)} & L1 & 2,882 & & Multiple Choice & Accuracy & Text only \\
\noalign{\vskip -1pt}\midrule\noalign{\vskip -1pt}
\multirow{5}{1.1cm}{\centering Alloy Materials}  & Alloy Chart QA & L2 & 15 &\checkmark& Multiple Choice & Accuracy & Chart \\
 & Composition Extraction & L2 & 244&\checkmark & Table Extraction & Table Accuracy & Table \\
 & Temperature Extraction & L2 & 207&\checkmark & Multiple Choice & Accuracy & Text only \\
 & Sample Differentiation & L3 & 237&\checkmark & Multiple Choice & Accuracy & Text only \\
 & Treatment Sequence & L3 & 102&\checkmark & True/False & Accuracy & Text only \\
 \noalign{\vskip -1pt}\midrule\noalign{\vskip -1pt}
 \multirow{6}{1.1cm}{\centering Biomedicine} 
 & Biology Chart QA & L2 & 99 &\checkmark& Multiple Choice & Accuracy & Chart \\
 & \textcolor{gray}{Chemical Entities Recognition} & L2 & 997 & & Text Extraction & Recall & Text only \\
 & \textcolor{gray}{Disease Entities Recognition} & L2 & 997 & & Text Extraction & Recall & Text only \\
 & \textcolor{gray}{Compound Disease Recognition} & L3 & 997 & & Text Extraction & Recall & Text only \\
 & \textcolor{gray}{Gene Disease Function} & L3 & 236 & & Text Extraction & Recall & Text only \\
 & \textcolor{gray}{Gene Disease Regulation} & L3 & 240 & & Text Extraction & Recall & Text only \\
\noalign{\vskip -1pt}\midrule\noalign{\vskip -1pt}
\multirow{7}{1.1cm}{\centering Drug Discovery} & Affinity Extraction & L2 & 40 &\checkmark& Table Extraction & Table Accuracy & Mol., Table \\
 & Drug Chart QA & L2 & 15 &\checkmark& Multiple Choice & Accuracy & Chart \\
 & Tag to Molecule & L2 & 50&\checkmark & Molecule Generation & Mol. Similarity & Mol. \\
 & Markush to Molecule & L3 & 37 & & Molecule Generation & Mol. Similarity & Mol. \\
 & Molecule in Document & L3 & 50 &\checkmark& True/False & Accuracy & Mol. \\
 & Reaction QA & L3 & 95 &\checkmark& Multiple Choice& Accuracy  & Reaction \\
 & Drug Target Identification & L3 & 40&\checkmark & Text Extraction & Recall & Text only \\
\noalign{\vskip -1pt}\midrule\noalign{\vskip -1pt}
\multirow{7}{1.1cm}{\centering Organic Materials} 
 & Electrolyte Table QA & L2 & 100 &\checkmark& Multiple Choice & Accuracy & Table \\
 & OLED Property Extraction & L2 & 13 &\checkmark& Table Extraction & Table Accuracy & Mol.,Table \\
 & Polymer Chart QA & L2 & 15 &\checkmark& Multiple Choice & Accuracy & Chart \\
 & Polymer Composition QA & L2 & 109 &\checkmark& Multiple Choice & Accuracy & Text only \\
 & Polymer Property Extraction & L2 & 109 &\checkmark& Table Extraction & Table Accuracy & Table \\
 & Solubility Extraction & L2 & 100 &\checkmark& Table Extraction & Table Accuracy & Table \\
 & Reaction Mechanism QA & L3 & 22 &\checkmark& Multiple Choice & Accuracy & Reaction\\
\bottomrule
\end{tabular}
\vspace{-4pt}
\caption{Statistics of the SciAssess. It comprises 14,721 questions across 29 tasks in five sub-domains. Tasks are categorized into three ability levels: Memorization (L1), Comprehension (L2), and Analysis \& Reasoning (L3). The context column denotes whether the task is based on given context from academic papers.
Tasks that are \textcolor{gray}{gray} are transformed from existing public datasets, while others are curated by domain experts hired by us.
}
\label{tab:benchmark-stat}
\vspace{-6pt}
\end{table*}

We begin by outlining the ability assessment framework in Section \ref{sec:ability_assess}, which serves as the backbone of our evaluation framework. 
Moving forward, we provide detailed description of evaluation scopes and tasks in Section \ref{sec:scope_and_task}.
Lastly, we present the quality control measures implemented to ensure the integrity and reliability in Section \ref{sec:data_compliance}.

\subsection{Ability Assessment Framework}\label{sec:ability_assess}
Guided by the widely accepted cognitive learning processes outlined in Bloom's Taxonomy \cite{taxonomy}, we propose that the evaluation of LLMs in scientific literature analysis should be classified into three core levels:

\textbf{Memorization (L1)} refers to the model's extensive knowledge base, which allows it to accurately answer common factual questions in science autonomously.
\textbf{Comprehension (L2)} is the ability to precisely identify and extract key information and facts within a given text, and to comprehend them.
\textbf{Analysis \& Reasoning (L3)} demonstrate the model's advanced capability to amalgamate extracted information with its existing knowledge base for logical reasoning and analysis, leading to well-founded conclusions or predictions.

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Memorization (L1)} refers to the model's extensive knowledge base, which allows it to accurately answer common factual questions in science autonomously.
    
%     \item \textbf{Comprehension (L2)} is the ability to precisely identify and extract key information and facts within a given text, and to comprehend them.
    
%     \item \textbf{Analysis \& Reasoning (L3)} demonstrate the model's advanced capability to amalgamate extracted information with its existing knowledge base for logical reasoning and analysis, leading to well-founded conclusions or predictions.
% \end{itemize}

Inspecting existing LLM benchmarks in science field (See Section \ref{sec:related_work}) through three-level ability assessment framework, we find that they mostly focus on Memorization (L1) -- the foundational knowledge base for scientific facts -- while overlooking the higher-level abilities of Comprehension (L2) and Analysis \& Reasoning (L3).

Given the significant potential of leveraging LLMs as scientific literature analysis assistants to boost scientific discovery, we propose SciAssess as a more comprehensive benchmark, in terms of tasks, scopes, and modalities.

% researchers and practitioners are now demanding a more suitable benchmark to help them select and optimize LLM-based scientific literature analysis assistants.

\subsection{Scope \& Task}\label{sec:scope_and_task}

After categorizing the ability of of LLMs into three levels, we proceed to introduce how we choose the tasks in SciAssess. As mentioned above, Memorization (L1), being the extensive foundation for other higher-level abilities, should encompass as large a knowledge base as possible. 
Therefore, SciAssess initially includes factual questions covering fundamental science subjects, such as chemistry, biology, \etc. 
For the evaluation of Comprehension (L2) and Analysis \& Reasoning (L3), we focus on vertical domains such as materials and biomedicine. 
The reason is that solving tasks in these domains require finer-grained abilities, such as understanding \textit{tables} and \textit{molecular structures}.
% , since the finer-grained ability requirements differ among these fields. 
For instance, crucial composition information in alloy material literature is often found in \textit{tables}, whereas key information extraction in drug discovery necessitates the accurate recognition of \textit{molecular structures}.
Thus, we further include four vertical domains: alloy materials, biomedicine, drug discovery, and organic materials, as shown in Figure \ref{fig:overview}. 
This categorization ensures that SciAssess captures the unique challenges and requirements of each specific field.

SciAssess, as presented in Table \ref{tab:benchmark-stat}, comprises 14,721 questions across 29 tasks in five scientific domain, encompassing three ability levels: Memorization (L1), Comprehension (L2), and Analysis \& Reasoning (L3). 
% This ensures a comprehensive evaluation of LLMs in scientific literature analysis.
Of these tasks, 19 out of 29 are based on contexts from academic papers, specifically designed to assess the ability to analyze scientific literature. 
We show the token lengths (GPT-4 tokenizer) of questions and answers for each task in Appendix \ref{app:length_distribution}.
SciAssess also includes five types of questions (\ie True/False questions, Multiple-Choice questions, Table Extraction, Text Extraction, and Molecule Generation) with four metrics (\ie accuracy, table recall, recall, molecule similarity).
For detailed descriptions and concrete examples, please refer to Appendix \ref{app:question-type}.
We also provide prompt template and specific prompt for each task in Appendix \ref{app:prompt-template} and \ref{app:task-prompt}, respectively.

% 通用化学领域
\subsubsection{Fundamental Science}
Aiming to evaluate foundational knowledge -- the basis of literature analysis, SciAssess should encompass as large a knowledge base as possible.
Several widely-adopted benchmarks could be leveraged to evaluate LLMs' awareness of commonsense facts across various domains.
Specifically, \textbf{MMLU} \cite{mmlu} consists of 57 tasks on various subjects, each containing multiple-choice questions that test domain-specific facts. 
\textbf{CMMLU} \cite{cmmlu} is a comprehensive Chinese benchmark that covers a wide range of 67 subjects. 
\textbf{Xiezhi} \cite{xiezhi} is a Chinese-English bilingual benchmark with 249,587 multiple-choice questions spanning 516 diverse disciplines. 
We filter out the STEM subsets, excluding mathematics, from these benchmarks and adapt them into a unified multi-choice template.
% This ensures a robust assessment of the models' foundational knowledge, which is crucial for their performance in scientific literature analysis.
A concrete example with prompt is provided in Appendix \ref{app:prompt-fundamental-science}.

% 合金领域
\subsubsection{Alloy Materials}

Alloy materials are composed of two or more metal elements mixed in specific proportions to exhibit metal-like characteristics. 
These materials are extensively used in aerospace, automobile manufacturing, construction, and other industries. 
By adjusting their composition and preparation processes, alloy materials can be tailored to meet specific properties and requirements \cite{caron1983improvement}. 
Thus, accurately extracting alloy composition and process parameters from literature is crucial for effective alloy design.

% In this domain, we evaluate the capabilities of LLMs in extracting key information for alloy design. 
% We have devised a comprehensive set of tasks related to literature research, which include extracting alloy composition, extracting process values, determining process sequences, and differentiating between samples. 
% The standard answers for all tasks have been manually extracted from literature across various journals and subsequently verified by an independent expert.

Specifically, following tasks are devised: \textbf{Alloy Chart QA}, \textbf{Composition Extraction}, \textbf{Temperature Extraction}, \textbf{Sample Differentiation}, and \textbf{Treatment Sequence}.
Detailed descriptions and prompt templates are provided in Appendix \ref{app:prompt-alloy-materials}.

% \textbf{Alloy Chart QA}
% \label{alloychartqa}
% The processing steps and properties of alloy materials are often presented in charts, such as those comparing the performance of multiple alloys or illustrating how elongation changes with composition. 
% Therefore, extracting information from these charts and integrating it with textual information is crucial. 
% To further evaluate the retrieval capability of models regarding alloy chart information, we have designed multiple-choice questions involving alloy composition, processing techniques, and properties.
% We prompt the model as in Appendix \ref{app:prompt-alloy-chart-qa}.

% \textbf{Composition Extraction}
% Extracting alloy composition information from an article's text or tables and unifying it into a structured format helps researchers utilize historical data more effectively and provides valuable guidance for subsequent designs. 
% This comprehensive task evaluates LLMs' ability to extract alloy compositions (including all element contents) from text and tables. 
% Typically, alloy element content is found in two cases: (1) the element content is stored in a table, and (2) the element content is implicitly indicated by the alloy name, such as `Fe30Co20Ni50', which represents an atomic ratio of 30\% Fe, 20\% Co, and 50\% Ni. 
% The objective of this task is to comprehensively extract this information and organize it into a digestible table.
% The metric is to calculate the matching score between the standard answer table and the extraction result table. 
% This task showcases the LLM's comprehension ability to integrate, extract, and structure multi-modal information \cite{kim2021prediction}.
% A concrete example is shown in Appendix \ref{app:prompt-composition-extraction}.

% \textbf{Temperature Extraction}
% The properties of an alloy are determined by its composition and the processes it undergoes, including processing and heat treatment. 
% Therefore, extracting heat treatment values is critical. 
% This task aims to determine the maximum temperature value for the heat treatment of the alloy. 
% To ensure easy statistical analysis, questions are designed as multiple-choice.
% An example and corresponding prompt are provided in Appendix \ref{app:prompt-temperature-extraction}.

% \textbf{Sample Differentiation}
% Alloys with the same composition but treated by different processes are considered different samples because they exhibit different properties. 
% Therefore, distinguishing between different samples and understanding the differences in their processes is essential. 
% This multiple-choice question task is designed to comprehensively judge the number of different alloy samples proposed or studied by the authors. 
% It assesses the LLMs' analysis and reasoning abilities regarding alloy distinctions from text.
% We show example context and prompt in Appendix \ref{app:prompt-sample-differentiation}.

% \textbf{Treatment Sequence}
% Each alloy treatment process has a clear sequence requirement, so it is necessary to ensure that the extracted heat treatment process sequence is consistent with the experimental sequence.
% For example, after solution treatment, a sample is further aged to ensure the release of internal stresses. 
% This task aims to objectively analyze and evaluate the sequential relationship between two heat treatments and provide True/False answers. 
% Additionally, if a specific heat treatment name does not exist in the paper, it should be considered False. 
% This task assesses the LLM's comprehension ability to judge treatment order from the text.

% It is worth noting that the definition of the alloy process steps is based on the complete heat treatment process, such as the two consecutive process steps (annealing and tempering); each step contains the temperature rise, constant temperature, and cooling stages. Under this definition, the previous process of tempering should be judged to be annealing, rather than annealing cooling sub-stages.
% Our prompt can be found in Appendix \ref{app:prompt-treatment-sequence}.

\subsubsection{Biomedicine} 


Biomedical literature encompasses a wealth of specialized terminology and complex concepts, as well as a significant amount of non-textual information such as tables and figures.
Effectively extracting and integrating these elements presents a crucial challenge. 
Given that tasks in the biomedical domain typically require precise identification and understanding of intricate biological entities, processes, and relationships, we have selected a set of representative tasks, including the recognition of specialized terminology, the comprehension of chart information, and the extraction of entity relationships, to evaluate the performance of LLMs in the biomedical field.

In this domain, following tasks are devised: \textbf{Biology Chart QA}, \textbf{Chemical Entities Recognition}, \textbf{Disease Entities Recognition}, \textbf{Compound Disease Recognition}, and \textbf{Gene Disease Function} \& \textbf{Gene Disease Regulation}.
Detailed descriptions and prompts are provided in Appendix \ref{app:prompt-biomedicine}.

% These tasks encompass key aspects of the biomedical domain, including the recognition of specialized terminology, the comprehension of graphical information, and the extraction of entity relationships. By addressing these diverse facets, the evaluation can provide a comprehensive assessment of large language models' capabilities in the biomedical domain, which in turn can inform further optimization and application of these models.

% \textbf{Biology Chart QA}
% The analysis and understanding of biological properties, compositions, and processing techniques are critical for the discovery and development in life sciences. 
% Often, this information is presented in charts, making it essential to extract and integrate such information with textual data. 
% To assess the retrieval capabilities of models in the context of biological chart information, we have designed multiple-choice questions.
% The example of biological ChartQA can be found in a similar format to the Alloy ChartQA task in Section~\ref{alloychartqa}.

% \textbf{Chemical Entities Recognition} 
% This task involves recognizing chemical entity names using data from B5CDR \cite{CDR2016} and additional expert-annotated data. It evaluates the performance of LLMs in identifying complex drug names.
% An example paragraph and corresponding prompt can be found in Appendix \ref{app:prompt-chemical-entities-recognition}.

% \textbf{Disease Entities Recognition} 
% Similarly, this task involves recognizing disease entity names using data from \cite{CDR2016} and additional expert-annotated data, evaluating the performance of LLMs in identifying specialized disease names.
% An example paragraph and corresponding prompt can be found in Appendix \ref{app:prompt-disease-entities-recognition}.

% \textbf{Compound Disease Recognition} 
% Proposed in B5CDR \cite{CDR2016}, this task evaluates the capability of LLMs to identify and understand associations between compounds and diseases. 
% An example paragraph and corresponding prompt can be found in Appendix \ref{app:prompt-compound-disease-recognition}.

% \textbf{Gene Disease Function} \& \textbf{Gene Disease Regulation}
% The Gene Disease Text Mining task focuses on "Gene-Disease" association semantics text mining. 
% It evaluates the ability of models to extract and understand relationships between genes and diseases from scientific literature, with a focus on identifying gene and disease entities \cite{GDAS2022}.

% In order to test the model's ability of text comprehension and triplet extraction, predefined entities and relationships are designed to capture complex biomedical interactions: (entities, relationship, entities).

% \textit{Entities} encompass molecular objects such as \textit{Disease}, \textit{Gene}, \textit{Protein}, and \textit{Enzyme}, each representing various biological components crucial for understanding molecular biology and genetics. Trigger word entities include \textit{Variation} (Var), indicating changes in DNA, RNA, proteins, or molecular structures; \textit{Molecular Physiological Activity} (MPA), referring to molecular-level activities like gene expression; \textbf{Interaction}, denoting connections between molecules or between molecules and cells; \textit{Pathway}, encompassing various biological pathways; \textit{Cell Physiological Activity} (CPA), representing activities at or above the cellular level, including responses and development; and regulatory terms such as \textit{Regulation} (Reg), \textit{Positive Regulation} (PosReg), and \textit{Negative Regulation} (NegReg), which indicate neutral, gain, or loss of function clues respectively. The \textit{relationships} defined include \textit{semantic roles}, like \textit{ThemeOf}, pointing from the main event (Theme) entity towards the current entity, and \textit{CauseOf}, directing from the current entity to the cause entity, as well as \textit{regulatory types} are categorized into \textit{LOF} (loss of function), \textit{GOF} (gain of function), \textit{REG} (general regulation), and \textit{COM} (complex functional changes between genes and diseases), aiming to predict "gene; function change; disease" triples from the text, illustrating the intricate dynamics between these biological entities and processes.

% The prompt for triplets (entities, semantic roles, entities) extraction is detailed in Appendix \ref{app:prompt-gene-disease-function}.

% \textbf{Gene Disease Regulation}
% The prompt for triplets (entities, semantic roles, entities) extraction is detailed in Appendix \ref{app:prompt-gene-disease-regulation}.

%药物发现领域
\subsubsection{Drug Discovery}

Drug discovery focuses on developing new therapeutics. 
Leveraging advanced intelligent tools, especially LLMs, can significantly enhance the efficiency and effectiveness of discovering and developing new drugs. 
These models are adept at parsing and analyzing complex data from diverse sources, including scientific texts and databases.

% We examine LLMs in drug discovery, setting out a series of tasks designed to evaluate their ability to extract and process key information from literature related to pharmacology and molecular biology. 
% These tasks aim to demonstrate how LLMs can be instrumental in identifying and understanding drug properties, interactions, and targets.

Specifically, we devise: \textbf{Affinity Extraction}, \textbf{Drug ChartQA}, \textbf{Tag to Molecule}, \textbf{Markush to Molecule}, \textbf{Molecule in Document}, \textbf{Reaction QA}, \textbf{Drug Target Extraction}.
Detailed descriptions and prompts are provided in Appendix \ref{app:prompt-drug-discovery}.
% \textcolor{blue}{The field of drug discovery-related literature encompasses a vast range of documents, including research papers, clinical trial reports, and patents, which are rich in specialized knowledge about drugs, chemical compounds, chemical reactions, biological mechanisms, and medical technology. Extracting accurate and useful information and constructing domain-specific datasets from these documents is critical for driving innovation in pharmacology, drug discovery, and therapy development. However, the intrinsic complexity of the data, characterized by specialized terminology, chemical structures, tables, and intricate relationships, poses significant challenges for information extraction.}

% \textcolor{blue}{In this chapter, we focus on information from novel molecules and the results of bioassays. The \textbf{Affinity Extraction} task is a comprehensive one that collects all the assay information and infers the molecule structures. The following tasks are subtasks of the first task and represent the logical steps necessary for its implementation.}

% \textbf{Affinity Extraction}
% This task evaluates the LLM's ability to extract an affinity table containing molecules' tags, SMILES, and their affinities to different targets in bioassays. 
% It tests several key capabilities of LLMs, including understanding complex and domain-specific language, as well as molecules and tables. 
% Affinity data extraction requires not just surface-level text processing but also a deeper analysis to match different modalities.

% The dataset is curated from \href{https://pubchem.ncbi.nlm.nih.gov/docs/bioassays}{PubChem BioAssays} to cover literature from different journals and years. Since the original dataset is organized by bio-assay numbers, we merge the source data according to their DOIs, and carefully sampled a subset of them. The papers have a large coverage of protein targets and cell lines, in the meanwhile have different display formats of the tables.
% We prompt LLM as in Appendix \ref{app:prompt-affinity-extraction}.

% \textbf{Drug Chart QA}
% The analysis of drug properties, compositions, and processing techniques is critical for drug discovery and development. 
% Often, this information is presented in charts, making it essential to extract and integrate such information with textual data. 
% To further assess the retrieval capabilities of models in the context of drug chart information, we have designed multiple-choice questions focusing on drug composition, processing methods, and properties. 
% The example of drug ChartQA can be found in a similar format to the Alloy ChartQA task in Section~\ref{alloychartqa}.

% \textbf{Tag to Molecule}
% This task evaluates the model's ability to find the correct SMILES given its tag in a document. 
% Typically, a molecule is shown with an chart of its structure and a tag below it. 
% The LLM should recognize both the structure and the tag and understand their connection.
% The detailed prompt for this task is provided in Appendix \ref{app:prompt-tag2molecule}.

% \textbf{Markush to Molecule}
% This task evaluates the model's ability to obtain the correct SMILES given a Markush formula (in CXSMILES pattern) and its substituents.
% We prompt LLM as in Appendix \ref{app:prompt-markush2molecule}.

% \textbf{Molecule in Document}
% This task evaluates the model's ability to determine whether a molecule (represented by SMILES) is mentioned in a document. 
% The LLM should recognize all Markush formulas and their substituents, and then judge whether the required molecule is covered.
% The prompt for this task can be found in Appendix \ref{app:prompt-molecule-in-doc}.

% \textbf{Reaction QA}
% Organic and bio-catalyzed synthetic reactions are vital for the manufacture of drug-like molecules. 
% Therefore, we designed a complex task to test the model's capability in extracting information from schematic diagrams and texts of chemical reactions. 
% The model is required to understand the charts specified in the articles and select the correct answer from the provided multiple-choice descriptions.
% We prompt LLM as in Appendix \ref{app:prompt-reaction-qa}.

% \textbf{Drug Target Extraction}
% This task evaluates the model's ability to find all related targets (proteins or cell lines) of the bioassays given a document.


% 有机材料领域
\subsubsection{Organic Materials}
Organic materials, derived from carbon-based molecules or polymers, exhibit distinct functionalities advantageous across a spectrum of applications. 
Distinguished from their inorganic counterparts by their modifiable properties and adaptability, these materials are vital in applications such as electronics, sensing, and energy. 
% They leverage the vast potential of organic chemistry for technological advancements.
In this section, we focus on two subfields within organic functional materials: organic electrolytes and polymer materials. 

We devise following tasks for organic materials: \textbf{Electrolyte Table QA}, \textbf{OLED Property Extraction}, \textbf{Polymer Chart QA}, \textbf{Polymer Composition Extraction}, \textbf{Polymer Property Extraction}, \textbf{Solubility Extraction}, \textbf{Reaction Mechanism QA}.
Detailed descriptions and prompt templates are provided in Appnedix \ref{app:organic-materials}.
% For polymer materials, we evaluate the efficacy of LLMs in extracting crucial properties associated with polymer materials from the scientific literature. 
% Specifically, we focus on the application of conjugated polymers in organic solar cells as a case study and design tasks to assess the model's ability to recognize and identify information about these materials.

% \textbf{Electrolyte Table QA}
% The composition and properties of organic electrolytes are crucial for battery performance, stability, and safety. To evaluate the model's retrieval capabilities regarding electrolyte information, we posed multiple-choice questions about the components of solution systems and the dissolution reactions, focusing on their physical and chemical properties as presented in the tables within the articles.
% Our prompt is detailed in Appendix \ref{app:prompt-electrolyte-table-qa}.


% \textbf{OLED Property Extraction}
% This task evaluates the LLM's ability to extract information about OLED molecules and their optical properties. 
% It tests several key capabilities, including their understanding of complex and domain-specific language and their ability to interpret and extract data from tables.
% A concrete example is provided in Appendix \ref{app:prompt-oled-property-extraction}.


% \textbf{Polymer Chart QA}
% The processing steps and properties of polymer materials are often represented through charts. 
% Extracting information from these charts and integrating it with textual data is crucial. 
% To further assess the retrieval capabilities of models concerning polymer chart information, we designed multiple-choice questions involving polymer composition, processing techniques, and properties.
% % The example of polymer ChartQA is similar to the Alloy ChartQA task in Section~\ref{alloychartqa}.

% \textbf{Polymer Composition Extraction} 
% This task involves extracting the blend ratio of donor to acceptor in the most efficient solar cell from the text of scientific literature. 
% By employing LLMs to extract these properties, we demonstrate significant potential for LLM in polymer modeling, including computer-aided screening, targeted design, and optimization. 
% Source data are collected from journals including \emph{Nature Communications, Advanced Materials, Nature Photonics, Nature Commun., J. Phys. Chem, J. Am. Chem. Soc. and Appl. Phys. Lett}.
% We detail the prompt in Appendix \ref{app:prompt-polymer-composition-extraction}.


% \textbf{Polymer Property Extraction} 
% This task focuses on extracting vital values such as power conversion efficiency (PCE) and open-circuit voltage ($V_{\mathrm{OC}}$) from tables within the literature. 
% By employing LLMs to extract these properties, we highlight significant potential for AI in polymer modeling, including computer-aided screening, targeted design, and optimization.
% Source data are collected from journals including \emph{Nature Communications, Advanced Materials, Nature Photonics, Nature Commun., J. Phys. Chem, and Appl. Phys. Lett}.
% We prompt LLM as in Appendix \ref{app:prompt-polymer-property-extraction}.

% \textbf{Solubility Extraction}
% Organic electrolytes, extensively used in battery technologies, comprise organic solvents, lithium salts, and additives. 
% Understanding solubility in organic electrolytes is crucial as it impacts the efficiency of electrolytic processes, product selectivity, and equipment design. 
% This task evaluates the LLM's capability in retrieving solubility-related tables. 
% Papers typically select data from various aspects to describe the system, making it challenging to combine multiple tables for fuzzy matching. 
% Therefore, we focus on examining the LLM's semantic understanding ability, enabling the model to select the most relevant and comprehensive table related to ``solubility'' from numerous alternatives and convert it into the specified format.
% Organic electrolytes are electrolytic solutions extensively used in battery technologies, especially in lithium-ion batteries. Comprising organic solvents, lithium salts, and additives when necessary, these electrolytes facilitate ion transfer within the battery, enabling energy storage and release. 

% Understanding solubility in organic electrolytes is crucial as it directly impacts the efficiency of electrolytic processes, product selectivity, and equipment design in various applications. In this task, we intend to investigate the LLM's capability in retrieving solubility-related tables. Considering the fact that papers related to the topic of electrolytes typically select data from various aspects to describe the system, requesting models combine multiple tables into an appropriate format for fuzzy matching turns out to be overly difficult. Therefore, we choose to focus more on examining the semantic understanding ability of LLMs, enabling the model to select the most relevant and largest table related to "solubility" from numerous alternatives and then converting it into the specified format.
% A concrete example can be found in Appendix \ref{app:prompt-solubility-extraction}.

% \textbf{Reaction Mechanism QA}
% Investigating electrolyte reactions helps improve the solid electrolyte interphase (SEI) layer, which directly affects battery performance and lifespan. 
% Studies in this area lead to the development of advanced electrolytes that enhance a robust SEI, resulting in more efficient and durable batteries. 
% We design a complex task to test the capability of extracting information from schematic diagrams of chemical reaction mechanisms. 
% LLM is required to understand the specified reaction diagram and select the correct answer from the provided multiple choices.
% Investigating electrolyte reactions helps improve the SEI layer, directly affecting battery performance and lifespan. Such studies lead to the development of advanced electrolytes that enhance a robust SEI, resulting in more efficient and durable batteries. Hence we designed a complex task to test the model's capability in extracting information from schematic diagrams of chemical reaction mechanisms. We require the model to understand the charts specified in the articles and select the correct answer from the provided multiple-choice descriptions.
% The prompt for this task can be found in Appendix \ref{app:prompt-reaction-mechanism-qa}.

\subsection{Data Quality, Privacy, and Copyright Compliance}\label{sec:data_compliance}
To safeguard the quality and ethical standards, meticulous steps were undertaken in its preparation and validation:

\textbf{Expert Validation:} 
Each original data point (as indicated by black tasks in Table \ref{tab:benchmark-stat}) is independently labeled by two annotators who are domain experts in the relevant fields.
If their labels agree, the label is accepted; if not, they engage in a discussion to determine the final label.

\textbf{Screening and Anonymization:} 
Our annotators were instructed not to use any data samples containing sensitive information when building the benchmark.
For example, data samples including personal health information or specific drug details were carefully reviewed. 
If such sensitive information was identified, it was either anonymized by removing personal identifiers or replacing specific details with general terms, or the entire sample was excluded from the benchmark.

\textbf{Copyright Compliance:} 
Our benchmark includes two types of data: some are adopted from existing benchmarks, and others are constructed from scratch by our team. 
For the data adopted from existing benchmarks, we provide the corresponding sources. 
For the data we created, we have obtained the necessary copyrights for the files used. 
To ensure full compliance with copyright laws, our repository only provides the Digital Object Identifier (DOI) for papers or patent number, and does not distribute the actual documents.
    

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Expert Validation:} 
%     Each original data point (as indicated by black tasks in Table \ref{tab:benchmark-stat}) is independently labeled by two annotators who are domain experts in the relevant fields.
%     If their labels agree, the label is accepted; if not, they engage in a discussion to determine the final label.

%     \item \textbf{Screening and Anonymization:} 
%     Our annotators were instructed not to use any data samples containing sensitive information when building the benchmark.
%     For example, data samples including personal health information or specific drug details were carefully reviewed. 
%     If such sensitive information was identified, it was either anonymized by removing personal identifiers or replacing specific details with general terms, or the entire sample was excluded from the benchmark.

%     \item \textbf{Copyright Compliance:} 
%     Our benchmark includes two types of data: some are adopted from existing benchmarks, and others are constructed from scratch by our team. 
%     For the data adopted from existing benchmarks, we provide the corresponding sources. 
%     For the data we created, we have obtained the necessary copyrights for the files used. 
%     To ensure full compliance with copyright laws, our repository only provides the Digital Object Identifier (DOI) for papers or patent number, and does not distribute the actual documents.
    
% \end{itemize}

